Towards model-independent exclusion of light Stops

Understanding the extent to which experimental searches are sensitive to Light Stops (LST) scenarios is essential to resolve questions about naturalness, electroweak baryogenesis and Dark Matter. In this paper we characterize the reach on LST scenarios in two ways. We extend experimental searches to cover specific gaps in the LST parameter space, showing for the first time that assuming a single decay channel one can exclude the region of $m_{\tilde{t}}<m_{top}$, which in its turn excludes electroweak baryogenesis in MSSM. Also, we explore the extent to which searches are weakened in a more generic scenario when more than one decay channel takes place, even after their combination. This study highlights the need for a more comprehensive exploration of the LST parameter space.

==> 1-Introduction-sasha.tex <==
\section{Introduction\label{sec:Intro}}

Supersymmetry (SUSY)~\cite{Golfand:1971iw,Ramond:1971gb,Neveu:1971rx,Gervais:1971ji,Volkov:1973ix,Wess:1973kz} is one of the most favoured theories beyond the Standard Model (SM).  It naturally solves the hierarchy problem, provides  gauge coupling unification and can address fundamental experimental problems of the SM on the cosmological scale, such as Dark Matter(DM) and Electroweak Baryogenesis. SUSY enlarges the SM spectrum of particles by their superpartners (sparticles), in particular with scalar partners of SM fermions -- sfermions. There are two scalar partners for each SM fermion, one corresponding to each chirality, conserving the number of degrees of freedom. Among them, stop quarks(stops), $\tilde{t}_{1,2}$, the super partners of the top-quark play a special role.

First of all $\tilde{t}_{1,2}$ controls the radiative corrections to the Higgs boson mass, measured to be around 125~GeV~\cite{CMS:2014ega,Aad:2014aba}. For the minimal supersymmetric standard model (MSSM) this implies  that the mass of at least one of  $\tilde{t}_{1,2}$ should be {\it of the order of above} a TeV scale, since radiative corrections are proportional to the  $\log$ of $\tilde{t}_{1,2}$, and are required to be large because the tree-level MSSM mass is below $M_Z$. 
This puts the mass of $\tilde{t}_{1,2}$ in tension with SUSY naturalness which suggests 
that the third generation squarks should be {\it below about 1 TeV}~\cite{Ellis:1986yg,Barbieri:1987fn}. This follows from the simple equation
\begin{equation}
\frac{M_Z^2}{2} \simeq M_{H_u}^2-\mu^2
\label{eq:ft}
\end{equation}
which connects the $Z$-boson mass, $M_Z$, the radiatively corrected $H_u$ mass term of the 
superpotential, $M_{H_u}$ (which depends on the stop contributions) and the superpotential higgsino mass, $\mu$.
It has however been shown that the usual fine-tuning measures, defined as the sensitivity of the weak scale to fractional variations in the fundamental parameters of the theory, can be low even if the masses of the supersymmetric scalars 
are large. 
This happens in the so called ``hyperbolic branch"(HB)~\cite{Chan:1997bi} or ``focus point" 
(FP)~\cite{Feng:1999mn,Feng:1999zg,Feng:2011aa} regions of the minimal super gravity (mSUGRA) parameter space, where the value of the Higgs mass parameter, $\mu$, can be low if the universal gaugino mass $M_{1/2}$ is not too large.
Moreover it was recently argued~\cite{Baer:2013gva} that EW fine-tuning in SUSY scenarios 
can be grossly overestimated by neglecting additional terms, stemming from the ultra violet (UV) completion of the model, that can lead
to large cancellations favouring a low $\mu$-parameter and allowing a heavier stop mass (up to a certain limit).


Besides its connection to the Higgs boson mass and fine-tuning,
the light stops can also affect the Higgs signal at the LHC, namely by altering its production via gluon-gluon fusion
and decay branching ratios, which was the subject of many detailed studies, see e.g.~\cite{Espinosa:2012in,Altmannshofer:2012ks,Carena:2013iba,Belyaev:2013rza,Fan:2014txa,Katz:2015uja} for light stops, Refs.~\cite{Henning:2014wua,Drozd:2015kva,Huo:2015nka} for studies in the context of Effective Field Theories, {and \cite{Belanger:2015vwa} for a study where flavour and Dark Matter constraints are also considered}.
In particular, it was shown~\cite{Belyaev:2013rza} that a scenario with light stops, would be able 
to explain a non-universal alteration of the two most relevant Higgs production channels ---
gluon-gluon fusion and vector boson fusion ones.


Finally, one should note that the light
stop scenario  is also attractive from a cosmological point of view. Firstly, there is a scenario where the lightest neutralino, being Dark Matter (DM) is degenerate with the lightest stop in the 100-300 GeV range, which predicts a plausibly low amount of DM (via the stop-neutralino co-annihilation channel)~\cite{Boehm:1999bj,Ellis:2001nx,Balazs:2004ae,Ellis:2014ipa,deSimone:2014pda}, and secondly the light stop scenario enables Electro-Weak Baryo-Genesis (EWBG) by facilitating a first-order phase transition, specifically requiring very
light stops ($m_{\tilde{t}}<150$~GeV)\cite{Carena:1997gx}.
{It should be noted that a number of papers claim to have ruled out light stop mediated EWBG in the MSSM by setting limits on stop masses using Higgs data \cite{Katz:2015uja,Cohen:2012zza,Curtin:2012aa}. However others have found loop holes in such arguments, such as the case where neutralinos have masses below about 60 GeV causing a sizeable Higgs decay to invisible \cite{Carena:2012np} or in the so-called {\it funnel region}~\cite{Espinosa:2012in} where the two stops could conspire to eliminate their effect on Higgs couplings. 
One should also note that the LST exclusion of 100 GeV stops using  the Higgs data
is substantially  weakened in case of  $m_{\tilde{t}}\simeq 150$~GeV
which still could possibly trigger EWSBG.
Therefore ruling out the existence of light stops via direct searches is an important step in 
straigthforward exclusion of  EWBG, as this way  is independent of Higgs measurements and closes  loopholes mentioned above.} 


One can see that the answer to the question of what is the lower stop mass limit is  
crucial for  different aspects of Supersymmetry -- one of the most appealing BSM theories. 
Currently the  light stops mass range below 300 GeV is  highly restricted by present experimental data, but 
not fully excluded. For example, the region near the thresholds of stop decay 
to  $Wb\tilde{\chi}^0$ or to  $t\tilde{\chi}^0$  has not been fully covered neither by ATLAS nor by  CMS collaborations.
This can be seen  from  ATLAS and CMS  combined limits on the stop mass in the neutralino-stop mass plane presented in Fig.~\ref{stop-atlas-cms}  which
is taken from  Refs.~\cite{atlas-stop,cms-stop}.
\begin{figure}[htb]
\includegraphics[width=0.62\textwidth]{ATLAS_stop}\\
\includegraphics[width=0.62\textwidth]{CMS-stst_2015}
\caption{Combined results on stop searches by ATLAS(top)~\cite{atlas-stop} and CM(bottom)~\cite{cms-stop} collaborations:
presenting the 95\% confidence limits (CL) exclusion region in the stop mass ($m_{\tilde{t}}$) vs neutralino mass ($m_{\tilde{\chi}^0_1}$) plane. Each search assumes a 100\% branching ratio via certain channels as shown in the legend of the plot
\cite{ATLAS_Twiki,Aad:2012ywa,Aad:2012xqa,Aad:2012uu,Aad:2014kra,Aad:2014bva,Aad:2014qaa,Aad:2014mfk,Aad:2014nra}.
\label{stop-atlas-cms}}
\end{figure}
%
From this figure one can see that indeed for the $\Delta m = m_{\tilde{t}}-m_{\tilde{\chi}^0_1} \gtrsim m_b+m_W$,
i.e. just below the line indicating the $Wb\tilde{\chi}^0$ threshold, there is a small sleeve of the allowed parameter space 
for  $m_{\tilde{t}}$ even below 150~GeV. 
{We should note that while finalising this paper we were made aware of a phenomenological paper \cite{Rolbiecki:2015lsa} which improves on the limits in this region using precision measurements of the $W^+ W^-$ cross section. Our approach is different and complimentary, and also more general as we explicitly consider also large branching ratios to the 2-body $\tilde{t}_1 \to c\tilde{\chi}^0_1$ final state.}

When $\Delta m <  m_b+m_W$, the stop can decay via a
radiatively induced $\tilde{t}_1 \to c\tilde{\chi}^0_1$ 2-body (2BD) flavour violating channel which can be large or even dominant in this  $\Delta m$ region. Moreover,  in the very narrow region
$m_c<\Delta m <  m_b$ (not indicated in Fig.~\ref{stop-atlas-cms}) this is the only possible decay channel. The other possible decay in the  $\Delta m <  m_b+m_W$
parameter space is the 4-body stop decay channel (4BD) $\tilde{t}_1 \to b f \bar{f'} \tilde{\chi}^0_1$,
were $f$ and $f'$ are either quarks of the 1st or 2nd generation, or leptons.
This decay is realised either via the exchange of a virtual top quark and W-boson and/or a virtual chargino.
In this paper we are interested in the LHC sensitivity to the light stop (LST)
scenario, which  we define hereafter as $m_{\tilde{t}}<m_{top}$ to be concrete.
One can see in Fig.~\ref{stop-atlas-cms} that the LST scenario can be 
excluded assuming a 100\% branching ratio to 2BD decays using monojet and 
charm-tagged monojet signals~\cite{Aad:2014nra} or under the assumption of a 100\% branching ratio to 4BD decay 
using a combination of monojet-like signal selection~\cite{Aad:2014nra} (which is also studied by CMS~\cite{CMS:2014yma}) and  single lepton plus missing transverse momentum signatures~\cite{Aad:2014kra}.
The very important question is the status of  the LST scenario
in the case of mixed branching ratios. This can be parameterised by a single parameter 
\begin{equation}
\epsilon_{2B}=Br(\tilde{t}_1 \to c\tilde{\chi}^0_1)
\end{equation}
so,
\begin{equation}
Br(\tilde{t}_1 \to b f \bar{f'} \tilde{\chi}^0_1) =1-\epsilon_{2B}.
\end{equation}
This is one of the objectives we study in our paper.
Indeed, this simple parameterisation is possible in the $\Delta m <  m_b+m_W$
region since no new kinematics is expected  in the form of on-shell lightest chargino decay since its mass is limited by LEPII 
to be above about 88 GeV\cite{Heister:2002mn,Barate:1997dr,Heister:2002vh,Barate:1999fs}, so $\Delta m <  m_b+m_W < m_{\tilde{\chi}^\pm_1}$.

In the  $ m_b+m_W < \Delta m <  m_t$  region
the model-independent exploration of LST scenario is much more complicated as it can
involve the new kinematics from  the on-shell chargino decay.
In general, one needs to involve two  more parameters in this region -- the chargino mass and 
the branching ratio of decay via the on-shell chargino,
$ Br(\tilde{t}_1 \to  b \tilde{\chi}^{\pm}_1 \to b W^{\ast} \tilde{\chi}^0_1)$.
This mass region was explored under different assumptions by ATLAS
using 1- and 2-lepton signatures\cite{Aad:2014kra,Aad:2014qaa} and CMS using a 1-lepton signature\cite{Chatrchyan:2013xna}
and a signature involving fully hadronic final states from stops decay~\cite{Khachatryan:2015wza}.
The CMS collaboration has parameterised chargino mass using a parameter $x$ $(0,1.)$
\begin{equation}
m_{\tilde{\chi}^\pm_1}=x m_{\tilde t} + (1-x) m_{\tilde{\chi}^0_1}
\end{equation}
which defines the ``position'' of the chargino  between the stop and the lightest neutralino.
ATLAS and CMS studies in the $ m_b+m_W < \Delta m <  m_t$  region involving different signatures are very complementary
and very comprehensive,
but unfortunately they do not give a definitive answer as to whether the LST scenario is excluded or not over the whole MSSM parameter space. For example, the CMS study of fully hadronic final states from stops decay~\cite{Khachatryan:2015wza}
clearly demonstrates the importance of this signature to exclude the LST scenario
as indicated in Fig.~\ref{stop-cms-alljets}.
%
\begin{figure}[htb]
\includegraphics[width=0.8\textwidth]{CMS-SUS-14001-Fig11.pdf}\\
\caption{Observed 95\% CL mass exclusion limit curves for top-squark pair production,
taken from Fig.11 of CMS SUS-14-001 paper\cite{Khachatryan:2015wza}
\label{stop-cms-alljets}}
\end{figure}
%
However, it's important to note that the results of this study are very model dependent:
when $Br(\tilde{t}\to b\tilde{\chi}^\pm_1) \equiv 1-Br(\tilde{t}\to t\tilde{\chi}^0_1) = 100\%$,
this search maximally excludes the $ m_b+m_W < \Delta m <  m_t$ 
region, while in the opposite case when $Br(\tilde{t}\to t\tilde{\chi}^0_1) = 100\%$ it leaves this
region intact. 

This happens because this study only considers 
on-shell top-quarks for $\tilde{t}\to t\tilde{\chi}^0_1$ decays which do not occur when $ m_b+m_W < \Delta m <  m_t$,
contrary to the $\tilde{t}\to b\tilde{\chi}^\pm_1$ decays for which the 
$\tilde{\chi}^\pm_1$ is always on-shell
since the mass gap between the chargino and neutralino was fixed at 5 GeV.

One can see that in order to perform a generic exploration
of the LST scenario one should complete the study of the respective space. As discussed above, this parameter space is three-dimensional  in $\Delta m <  m_b+m_W$ region
($m_{\tilde{t}}, m_{\tilde{\chi}^0_1}$ and $\epsilon_{2B}$),  
and five-dimensional in the  $ m_b+m_W < \Delta m <  m_t$ region
($m_{\tilde{t}}, m_{\tilde{\chi}^0_1}, \epsilon_{2B}, m_{\tilde{\chi}^\pm_1}$ and $ Br(\tilde{t}_1 \to  b \tilde{\chi}^{\pm}_1 \to b W^{\ast} \tilde{\chi}^0_1)$).
One can see that a model-independent exploration of the LST scenario is quite a complicated task.
On the way towards completing this task we make a simplification and consider only the part of the LST parameter space 
assuming that the chargino is heavier than the stop: $ m_{\tilde{\chi}^\pm_1}>m_{\tilde{t}}$.
This assumption allows us to conveniently work in a three-dimensional space in both the
$\Delta m <  m_b+m_W$ and  $ m_b+m_W < \Delta m <  m_t$ cases i.e. in the whole LST parameter space.
Relaxing this assumption would be the topic of future work, and in what follows we assume $ m_{\tilde{\chi}^\pm_1}>m_{\tilde{t}}$.

In this paper we explore the full LST
parameter space ($m_{\tilde{t}}, m_{\tilde{\chi}^0_1}$ and $\epsilon_{2B}$)
(under the $m_{\tilde{\chi}^\pm_1}>m_{\tilde{t}}$ assumption) using simulations with stops decaying via an off-shell top-quark and a W-boson
and recasting existing ATLAS and CMS searches. This allows us to explore the RUN1 LHC sensitivity to the full LST parameter space which is the main new  result of this paper.
It is clear that the potential exclusion of the whole LST parameter space
would have a dramatic consequences for the  EWBG scenario and important 
connections to Higgs phenomenology.

%\AB{Todo:
%\\
%1. review Maggie papers
%\\
%2. Write about the improvement we did
%-- the exact ME simulation
%to cover difficult region, which makes the link to model-independent 
%coverage of the  $\Delta M$ parameter space.
%\\
%3. that we reproduce Exp results and go further establishing ours;
%that we made an attemt to understand the reson of the existing gaps and 
%aimed to improve the present experimental interpretation,
%making path towards mode-independent coverage $\Delta M$ parameter space
%Notes:
%ATLAS: 
%}

The rest of the paper is organised as follows.
In Section II we discuss the stop decay channels and their dependence on the MSSM parameters.
We continue in Section III to discuss experimental analyses for the 2BD $\tilde{t}_1 \to c\tilde{\chi}^0_1$,
and 4BD $\tilde{t}_1 \to b f \bar{f'} \tilde{\chi}^0_1$ channels, and the tools and framework with which 
we extend these.
In section IV we present our results on the extension of the current experimental analyses and demonstrate that
for a generic case with intermediate branching ratios to the 2BD and 4BD decays, the current stop mass
limits are drastically reduced.
We draw our conclusions it Section V.



